Provenance-Based Assessment of Plans in Context

Many real-world planning domains involve diverse information sources, external entities, and variable-reliability agents, all of which may impact the confidence, risk, and sensitivity of plans. Humans reviewing a plan may lack context about these factors; however, this information is available during the domain generation, which means it can also be interwoven into the planner and its resulting plans. This paper presents a provenance-based approach to explaining automated plans. Our approach (1) extends the SHOP3 HTN planner to generate dependency information, (2) transforms the dependency information into an established PROV-O representation, and (3) uses graph propagation and TMS-inspired algorithms to support dynamic and counter-factual assessment of information flow, confidence, and support. We qualified our approach's explanatory scope with respect to explanation targets from the automated planning literature and the information analysis literature, and we demonstrate its ability to assess a plan's pertinence, sensitivity, risk, assumption support, diversity, and relative confidence.

==> experiments.tex <==


\section{Examples}
\label{sec:experiments}
\label{sec:examples}

\hide{
\begin{figure*}
  \begin{center}
  % \includegraphics[width=\textwidth]{figures/ss-rover-plan.png}
  % \caption{Plan to acquire imagery with agent \textbf{Rover0}.}
  % \label{fig:ss-rover-plan}
  % \vspace{.2in}
  \includegraphics[width=\textwidth]{figures/ss-rover-plan-colored.png}
  \caption{A plan to acquire high-res imagery of \textbf{objective1} using the agent \textbf{rover0}.
  Color of links indicate information source reliability propagated from appraised sources (e.g., \textbf{Elevation Map} and \textbf{Terrain Map}) as an estimate of information support.
  The final action (at right) is a junction of high- and low-reliability sources.}
  \label{fig:ss-rover-plan-colored}
  \vspace{.2in}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-refute-rover-navigate.png}}
  \caption{Same plan as \figref{ss-rover-plan-colored}, after \textit{refuting} the \textbf{navigate} capability, by un-checking it at right.}
  \label{fig:ss-refute-rover-navigate}
  \end{center}
\end{figure*}
}

\begin{figure*}
  \begin{center}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-compare.png}}
  \caption{Provenance of the goal to acquire high-res imagery of \textbf{objective1}, which can be acquired through two different planned action sequences.}
  \label{fig:ss-compare}
  \end{center}
\end{figure*}

\begin{figure*}
  \begin{center}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-impact-take-image.pdf}}
  \caption{Viewing the relevance and reachability of the \textbf{take-image} action, including the sources it relies on, and the impact on downstream actions.}
  \label{fig:ss-impact-take-image}
  \end{center}
\end{figure*}

\hide{
\begin{figure*}
  \begin{center}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-refute-take-image.pdf}}
  \caption{Assessing the necessity of the \textbf{take-image} action by refuting it (at right) and observing downstream effects.}
  \label{fig:ss-refute-take-image}
  \end{center}
\end{figure*}}

\begin{figure*}
  \begin{center}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-refute-flier.pdf}}
  \caption{Counter-factually refuting an entire agent \textbf{flier1},
  and noting that the goal can still be achieved by \textbf{rover0}, but with less source reliability.}
  \label{fig:ss-refute-flier}
  \end{center}
\end{figure*}

\begin{figure*}
  \begin{center}
  \frame{
  \includegraphics[width=\textwidth]{figures/ss-refute-terrain-map.pdf}}
  \caption{Counter-factually refuting the \textbf{Terrain Map} information source to assess sensitivity.
  The action sequence with \textbf{rover0} is no longer possible.}
  \label{fig:ss-refute-terrain-map}
  \end{center}
\end{figure*}

